Planet Hunters TESS IV: A massive, compact hierarchical triple star system TIC 470710327

We report the discovery and analysis of a massive, compact, hierarchical triple system (TIC 470710327) initially identified by citizen scientists in data obtained by NASA's Transiting Exoplanet Survey Satellite (TESS). Spectroscopic follow-up observations obtained with the HERMES spectrograph, combined with eclipse timing variations (ETVs), confirm that the system is comprised of three OB stars, with a compact 1.10 d eclipsing binary and a non-eclipsing tertiary on a 52.04 d orbit. Dynamical modelling of the system (from radial velocity and ETVs) reveal a rare configuration wherein the tertiary star (O9.5-B0.5V; 14-17 M$_{\odot}$) is more massive than the combined mass of the inner binary (10.9-13.2 M$_{\odot}$). Given the high mass of the tertiary, we predict that this system will undergo multiple phases of mass transfer in the future, and likely end up as a double neutron star gravitational wave progenitor or an exotic Thorne-Zytkow object. Further observational characterisation of this system promises constraints on both formation scenarios of massive stars as well as their exotic evolutionary end-products.

==> Soetkin_refs.tex <==
@INPROCEEDINGS{Castelli_2003,
       author = {{Castelli}, F. and {Kurucz}, R.~L.},
        title = "{New Grids of ATLAS9 Model Atmospheres}",
     keywords = {Astrophysics},
    booktitle = {Modelling of Stellar Atmospheres},
         year = 2003,
       editor = {{Piskunov}, N. and {Weiss}, W.~W. and {Gray}, D.~F.},
       volume = {210},
        month = jan,
        pages = {A20},
archivePrefix = {arXiv},
       eprint = {astro-ph/0405087},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003IAUS..210P.A20C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MISC{ Zacharias_2012, 
author = {Zacharias N., Finch C.T., Girard T.M., Henden A., Bartlett J.L., Monet D.G., Zacharias M.I.}, 
title = "{VizieR Online Data Catalog: UCAC4 Catalogue}", 
year = "2012", 
eid = {I/322A}, 
}

@MISC{Cutri_2013, 
author = {Cutri R.M., Wright E.L., Conrow T., Fowler J.W., Eisenhardt P.R.M., Grillmair C., Kirkpatrick J.D., Masci F., McCallon H.L., Wheelock S.L., Fajardo-Acosta S., Yan L., Benford D., Harbut M., Jarrett T., Lake S., Leisawitz D., Ressler M.E., Stanford S.A., Tsai C.-W., Liu F., Helou G., Mainzer A., Gettngs D., Gonzalez A., Hoffman D., Marsh K.A., Padgett D., Skrutskie M.F., Beck R., Papin M., Wittman M.}, 
title = "{VizieR Online Data Catalog: AllWISE Data Release}", 
year = "2013", 
eid = {II/328}, 
}


@MISC{Henden_2016, 
author = {Henden A.A., Templeton M., Terrell D., Smith T.C., Levine S., Welch D.}, 
title = "{VizieR Online Data Catalog: AAVSO Photometric All Sky Survey (APASS) DR9}", 
year = "2016", 
eid = {II/336}, 
}


@ARTICLE{Reed_2003,
       author = {{Reed}, B. Cameron},
        title = "{Catalog of Galactic OB Stars}",
      journal = {\aj},
     keywords = {Catalogs, Stars: Early-Type},
         year = 2003,
        month = may,
       volume = {125},
       number = {5},
        pages = {2531-2533},
          doi = {10.1086/374771},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003AJ....125.2531R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MISC{Altmann_2017, 
author = {Altmann M., Roeser S., Demleitner M., Bastian U., Schilbach E.}, 
title = "{VizieR Online Data Catalog: Hot Stuff for One Year (HSOY)}",
year = "2017", 
eid = {I/339}, 
}

@MISC{Ammons_2006, 
author = {Ammons S.M., Robinson S.E., Strader J., Laughlin G., Fischer D., Wolf A.}, 
title = "{VizieR Online Data Catalog: Teff and metallicities for Tycho-2 stars}", 
year = "2006", 
eid = {V/136}, 
}

@MISC{Bourges_2017, 
author = {Bourges L., Mella G., Lafrasse S., Duvert G., Chelli A., Le Bouquin J.-B., Delfosse X., Chesneau O.}, 
title = "{VizieR Online Data Catalog: JMMC Stellar Diameters Catalogue - JSDC. Version 2}", 
year = "2017", 
eid = {II/346}, 
}


@MISC{Fabricius_2002, 
author = {Fabricius C., Hog E., Makarov V.V., Mason B.D., Wycoff G.L., Urban S.E.}, 
title = "{VizieR Online Data Catalog: Tycho Double Star Catalogue   (TDSC)}", 
year = "2002", 
eid = {I/276}, 
}


@MISC{Nascimbeni_2016, 
author = {Nascimbeni V., Piotto G., Ortolani S., Giuffrida G., Marrese P.M., Magrin D., Ragazzoni R., Pagano I., Rauer H., Cabrera J., Pollacco D., Heras A.M., Deleuil M., Gizon L., Granata V.}, 
title = "{VizieR Online Data Catalog: All-sky catalog of solar-type dwarfs}", 
year = "2016", 
eid = {J/MNRAS/463/4210}, 
journal = {\mnras}
}

@MISC{Lasker_2006, 
author = {Lasker B., Lattanzi M.G., McLean B.J., et al.}, 
title = "{VizieR Online Data Catalog: The Guide Star Catalog, Version 2.3.2   (GSC2.3)}", 
year = "2006", 
eid = {I/305}, 
}

@MISC{Droege_2007, 
author = {Droege, T. F., Richmond, M. W., Sallman, M.}, 
title = "{VizieR Online Data Catalog: TASS Mark IV patches photometric catalog, version 2}", 
year = "2007", 
eid = {II/271A}, 
}

@MISC{Cutri_2003, 
author = {Cutri R.M., Skrutskie M.F., Van Dyk S., Beichman C.A., Carpenter J.M., Chester T., Cambresy L., Evans T., Fowler J., Gizis J., Howard E., Huchra J., Jarrett T., Kopan E.L., Kirkpatrick J.D., Light R.M, Marsh K.A., McCallon H., Schneider S., Stiening R., Sykes M., Weinberg M., Wheaton W.A., Wheelock S., Zacarias N.}, 
title = "{VizieR Online Data Catalog: 2MASS All-Sky Catalog of Point Sources}", 
year = "2003", 
eid = {II/246}, 
}

@MISC{Altmann_2017, 
author = {Altmann M., Roeser S., Demleitner M., Bastian U., Schilbach E.}, 
title = "{VizieR Online Data Catalog: Hot Stuff for One Year (HSOY)}",
year = "2017", 
eid = {I/339}, 
}

@MISC{ Zacharias_2012, 
author = {Zacharias N., Finch C.T., Girard T.M., Henden A., Bartlett J.L., Monet D.G., Zacharias M.I.}, 
title = "{VizieR Online Data Catalog: UCAC4 Catalogue}", 
year = "2012", 
eid = {I/322A}, 
}

@MISC{Cutri_2013, 
author = {Cutri R.M., Wright E.L., Conrow T., Fowler J.W., Eisenhardt P.R.M., Grillmair C., Kirkpatrick J.D., Masci F., McCallon H.L., Wheelock S.L., Fajardo-Acosta S., Yan L., Benford D., Harbut M., Jarrett T., Lake S., Leisawitz D., Ressler M.E., Stanford S.A., Tsai C.-W., Liu F., Helou G., Mainzer A., Gettngs D., Gonzalez A., Hoffman D., Marsh K.A., Padgett D., Skrutskie M.F., Beck R., Papin M., Wittman M.}, 
title = "{VizieR Online Data Catalog: AllWISE Data Release}", 
year = "2013", 
eid = {II/328}, 
}


% @misc{2003Castelli,
%   title={Proc. IAU Symp.},
%   author={Castelli, F and Kurucz, RL and Piskunov, N and Weiss, WW and Gray, DF},
%   journal={Modelling of Stellar Atmospheres},
%   volume={210},
%   pages={20},
%   year={2003},
%   publisher={Cambridge Univ. Press}
% }


==> Table_results_Soetkin.tex <==
\begin{table*}
%\begin{adjustwidth}{-.5in}{-.5in}
%\renewcommand{\arraystretch}{1.1}
    \centering
 % \begin{threeparttable}
    \caption{Masses, effective temperatures, and contributions of the four fitted components, obtained from the SED fitting. Subscript `OB' is for the O9.5-B0.5V star, subscript `1' and `2' for the primary and secondary of the binary, respectivey, and `out' is for the outer 0.5" component. The contribution of the latter is always fixed to 23\% and is not tabulated.}
     \begin{tabular}{cccccccccccc}
        \hline \hline
        $M_{\text{OB}}$  & $T_{\text{eff,OB}}$ & $f_{\text{OB}}/f_{\text{tot}}$ & $f_{\text{1}}/f_{\text{tot}}$ & $f_{\text{2}}/f_{\text{tot}}$ &  $T_{\text{eff,1}}$ & $T_{\text{eff,2}}$ & $T_{\text{eff,out}}$  & $M_{\text{1}}$  & $M_{\text{2}}$ & $M_{\text{out}}$ \\
        
        [$M_{\odot}$] & [kK]&[\%]&  [\%]&  [\%]&  [kK]& [kK]&  [kK] &  [$M_{\odot}$] &[$M_{\odot}$] & [$M_{\odot}$]\\
        \hline
        14.0 & 28 & 65.45 & 9.24 & 2.31 & 12 & 11 & 15 - 25&8.5& 2.5& 14.4 - 6.1 \\
        14.0 & 28 & 65.45 & 10.01&1.54 & 12 & 11 & 15 - 25&9.2& 1.7& 14.4 - 6.1 \\
        14.0 & 28 & 66.22 & 7.70 & 3.08 & 12 & 10 & 15 - 25 & 7.0 & 4.0 & 14.2 - 6.0\\
        14.0 & 28 & 66.99 & 8.47& 1.54 & 11 & 10 & 15 - 25 & 9.0 & 2.0 & 14.0 - 5.9\\
        % 14.5 & 28 & 65.45 & 9.24 & 2.31 & 12 & 11 & 15 - 25&8.9& 2.6& 14.9 - 6.3 \\
        % 14.5 & 28 & 65.45 & 10.01&1.54 & 12 & 11 & 15 - 25&9.5& 1.7& 14.9 - 6.3 \\
        % 14.5 & 28 & 66.22 & 7.70 & 3.08 & 12 & 10 & 15 - 25 & 7.2 & 4.1 & 14.7 - 6.2\\
        % 14.5 & 28 & 66.99 & 8.47& 1.54 & 11 & 10 & 15 - 25 & 9.3 & 2.0 & 14.5 - 6.2\\
        15.0 & 28 & 65.45 & 9.24 & 2.31 & 12 & 11 & 15 - 25&9.1& 2.7& 15.4 - 6.5 \\
        15.0 & 28 & 65.45 & 10.01&1.54 & 12 & 11 & 15 - 25&9.8& 1.8& 15.4 - 6.5 \\
        15.0 & 28 & 66.22 & 7.70 & 3.08 & 12 & 10 & 15 - 25 & 7.5 & 4.3 & 15.2 - 6.4\\
        15.0 & 28 & 66.99 & 8.47& 1.54 & 11 & 10 & 15 - 25 & 9.6 & 2.1 & 15.0 - 6.4\\
        % 15.5 & 28 & 65.45 & 9.24 & 2.31 & 12 & 11 & 15 - 25&9.4& 2.8& 15.9 - 6.7 \\
        % 15.5 & 28 & 65.45 & 10.01&1.54 & 12 & 11 & 15 - 25&10.2& 1.8& 15.9 - 6.7 \\
        % 15.5 & 28 & 66.22 & 7.70 & 3.08 & 12 & 10 & 15 - 25 & 7.7 & 4.4 & 15.7 - 6.7\\
        % 15.5 & 28 & 66.99 & 8.47& 1.54 & 11 & 10 & 15 - 25 & 9.9 & 2.2 & 15.5 - 6.6\\
        16.0 & 28 & 65.45 & 9.24 & 2.31 & 12 & 11 & 15 - 25&9.7& 2.7& 16.4 - 7.0 \\
        16.0 & 28 & 65.45 & 10.01&1.54 & 12 & 11 & 15 - 25&10.5& 1.9& 16.4 - 7.0 \\
        16.0 & 28 & 66.22 & 7.70 & 3.08 & 12 & 10 & 15 - 25 & 8.0& 4.6 & 16.2 - 6.9\\
        16.0 & 28 & 66.99 & 8.47& 1.54 & 11 & 10 & 15 - 25 & 10.2 & 2.3 & 16.0 - 6.8\\
        % 16.5 & 28 & 65.45 & 9.24 & 2.31 & 12 & 11 & 15 - 25&10.0& 3.0& 16.9 - 7.2 \\
        % 16.5 & 28 & 65.45 & 10.01&1.54 & 12 & 11 & 15 - 25&10.8& 2.0& 16.9 - 7.2 \\
        % 16.5 & 28 & 66.22 & 7.70 & 3.08 & 12 & 10 & 15 - 25 & 8.2 & 4.7 & 16.7 - 7.1\\
        % 16.5 & 28 & 66.99 & 8.47& 1.54 & 11 & 10 & 15 - 25 & 10.6 & 2.3 & 16.5 - 7.0\\
        17.0 & 28 & 65.45 & 9.24 & 2.31 & 12 & 11 & 15 - 25&10.3& 3.0& 17.4 - 7.4 \\
        17.0 & 28 & 65.45 & 10.01&1.54 & 12 & 11 & 15 - 25&11.2& 2.0& 17.4 - 7.4 \\
        17.0 & 28 & 66.22 & 7.70 & 3.08 & 12 & 10 & 15 - 25 & 8.5& 4.9 & 17.2 - 7.3\\
        17.0 & 28 & 66.99 & 8.47& 1.54 & 11 & 10 & 15 - 25 & 10.9 & 2.4 & 17.0 - 7.2\\
       \hline
%      \end{tabular}
%          \flushleft
%     \begin{tablenotes}
%       \small
%       \item \textbf{Notes.} 
%     \end{tablenotes}
%     \label{table_28000K}
% %  \end{threeparttable}
% %\end{adjustwidth}
% \end{table*}


% \begin{table*}
% %\begin{adjustwidth}{-.5in}{-.5in}
% %\renewcommand{\arraystretch}{1.1}
%     \centering
%  % \begin{threeparttable}
%     \caption{The coontribution of the outer 0.5" component is always fixed to 23\%.}
%      \begin{tabular}{cccccccccccc}
%         \hline \hline
        % $M_{\text{OB}}$  & $T_{\text{eff,OB}}$ & $f_{\text{OB}}/f_{\text{tot}}$ & $f_{\text{1}}/f_{\text{tot}}$ & $f_{\text{2}}/f_{\text{tot}}$ &  $T_{\text{eff,1}}$ & $T_{\text{eff,2}}$ & $T_{\text{eff,out}}$  & $M_{\text{1}}$  & $M_{\text{2}}$ & $M_{\text{out}}$ \\
        
        % [$M_{\odot}$] & [kK]&[\%]&  [\%]&  [\%]&  [kK]& [kK]&  [kK] &  [$M_{\odot}$] &[$M_{\odot}$] & [$M_{\odot}$]\\
        % \hline
        14.0 & 29 & 65.45 & 8.47 & 3.08 & 13 & 11 & 15 - 25&7.2& 3.4& 15.4 - 6.5 \\
        14.0 & 29 & 66.22 & 7.70&3.08 & 13 & 10 & 15 - 25&6.5& 4.3& 15.3 - 6.5 \\
        14.0 & 29 & 66.22 & 8.47 & 2.31 & 12 & 11 & 15 - 25 & 8.3 & 2.7 & 15.3 - 6.5\\
        14.0 & 29 & 66.99 & 6.93& 3.08 & 12 & 10 & 15 - 25 & 6.7 & 4.2 & 15.1 - 6.4\\
        14.0 & 29 & 67.76 & 6.93& 2.31 & 11 & 10 & 15 - 25 & 7.8 & 3.1 & 14.9 - 6.3\\
        % 14.5 & 29 & 65.45 & 8.47 & 3.08 & 13 & 11 & 15 - 25&7.5& 3.7& 16.0 - 6.8 \\
        % 14.5 & 29 & 66.22 & 7.70&3.08 & 13 & 10 & 15 - 25&6.7& 4.4& 15.8 - 6.7 \\
        % 14.5 & 29 & 66.22 & 8.47 & 2.31 & 12 & 11 & 15 - 25 & 8.5 & 2.8 & 15.8 - 6.7\\
        % 14.5 & 29 & 66.99 & 6.93& 3.08 & 12 & 10 & 15 - 25 & 6.9 & 4.4 & 15.6 - 6.6\\
        % 14.5 & 29 & 67.76 & 6.93& 2.31 & 11 & 10 & 15 - 25 &8.1 & 3.4 & 15.4 - 6.5\\
        15.0 & 29 & 65.45 & 8.47 & 3.08 & 13 & 11 & 15 - 25&7.7& 3.8& 16.5 - 7.0 \\
        15.0 & 29 & 66.22 & 7.70&3.08 & 13 & 10 & 15 - 25&7.0& 4.6& 16.3 - 6.9 \\
        15.0 & 29 & 66.22 & 8.47 & 2.31 & 12 & 11 & 15 - 25 & 8.8 & 2.8 & 16.3 - 6.9\\
        15.0 & 29 & 66.99 & 6.93& 3.08 & 12 & 10 & 15 - 25 & 7.2 & 4.5 & 16.2 - 6.8\\
        15.0 & 29 & 67.76 & 6.93& 2.31 & 11 & 10 & 15 - 25 & 8.3 & 3.4 & 16.0 - 6.8\\
        % 15.5 & 29 & 65.45 & 9.24 & 2.31 & 12 & 11 & 15 - 25&9.4& 2.8& 15.9 - 6.7 \\
        % 15.5 & 29 & 65.45 & 10.01&1.54 & 12 & 11 & 15 - 25&10.2& 1.8& 15.9 - 6.7 \\
        % 15.5 & 29 & 66.22 & 7.70 & 3.08 & 12 & 10 & 15 - 25 & 7.7 & 4.4 & 15.7 - 6.7\\
        % 15.5 & 29 & 66.99 & 8.47& 1.54 & 11 & 10 & 15 - 25 & 9.9 & 2.2 & 15.5 - 6.6\\
        16.0 & 29 & 65.45 & 8.47 & 3.08 & 13 & 11 & 15 - 25&8.3& 4.1& 17.6 - 7.5 \\
        16.0 & 29 & 66.22 & 7.70&3.08 & 13 & 10 & 15 - 25&7.4& 4.9& 17.4 - 7.4 \\
        16.0 & 29 & 66.22 & 8.47 & 2.31 & 12 & 11 & 15 - 25 & 9.4 & 3.0 & 17.4 - 7.4\\
        16.0 & 29 & 66.99 & 6.93& 3.08 & 12 & 10 & 15 - 25 & 7.6 & 4.9 & 17.2 - 7.3\\
        16.0 & 29 & 67.76 & 6.93& 2.31 & 11 & 10 & 15 - 25 & 8.9 & 3.6 & 17.0 - 7.2\\
        % 16.5 & 29 & 65.45 & 9.24 & 2.31 & 12 & 11 & 15 - 25&10.0& 3.0& 16.9 - 7.2 \\
        % 16.5 & 29 & 65.45 & 10.01&1.54 & 12 & 11 & 15 - 25&10.8& 2.0& 16.9 - 7.2 \\
        % 16.5 & 29 & 66.22 & 7.70 & 3.08 & 12 & 10 & 15 - 25 & 8.2 & 4.7 & 16.7 - 7.1\\
        % 16.5 & 29 & 66.99 & 8.47& 1.54 & 11 & 10 & 15 - 25 & 10.6 & 2.3 & 16.5 - 7.0\\
        17.0 & 29 & 65.45 & 8.47 & 3.08 & 13 & 11 & 15 - 25&8.8& 4.4& 18.7 - 7.9 \\
        17.0 & 29 & 66.22 & 7.70&3.08 & 13 & 10 & 15 - 25&7.9& 5.2& 18.5 - 7.8 \\
        17.0 & 29 & 66.22 & 8.47 & 2.31 & 12 & 11 & 15 - 25 & 10.0 & 3.2 & 18.5 - 7.8\\
        17.0 & 29 & 66.99 & 6.93& 3.08 & 12 & 10 & 15 - 25 & 8.1 & 5.2 & 18.3 - 7.8\\
        17.0 & 29 & 67.76 & 6.93& 2.31 & 11 & 10 & 15 - 25 & 9.5 & 3.8 & 18.1 - 7.7\\
       \hline
        14.0 & 30 & 65.45 & 9.24 & 2.31 & 13 & 12 & 15 - 25&8.5& 2.4& 16.6 - 7.0 \\
        14.0 & 30 & 65.45 & 9.24 & 2.31 & 14 & 10 & 15 - 25&7.5& 3.5& 16.6 - 7.0 \\
        14.0 & 30 & 65.45 & 10.01 & 1.54 & 13 & 12 & 15 - 25 & 9.2 & 1.6 & 16.6 - 7.0\\
        14.0 & 30 & 66.99 & 6.93& 3.08 & 12 & 11 & 15 - 25 & 7.2 & 3.8 & 16.2 - 6.9\\
        14.0 & 30 & 66.99 & 7.70& 2.31 & 12 & 11 & 15 - 25 & 8.0 & 2.8 & 16.2 - 6.9\\
        14.0 & 30 & 67.76 & 6.16& 3.08 & 12 & 10 & 15 - 25 & 6.3 & 4.5 & 16.0 - 6.8\\
        14.0 & 30 & 68.53 & 5.39& 3.08 & 11 & 10 & 15 - 25 & 6.4 & 4.5 & 15.8 - 6.7\\
         15.0 & 30 & 65.45 & 9.24 & 2.31 & 13 & 12 & 15 - 25&9.1& 2.6& 17.7 - 7.5 \\
        15.0 & 30 & 65.45 & 9.24 & 2.31 & 14 & 10 & 15 - 25&8.0& 3.7& 17.7 - 7.5 \\
        15.0 & 30 & 65.45 & 10.01 & 1.54 & 13 & 12 & 15 - 25 & 9.8 & 1.7 & 17.7 - 7.5\\
        15.0 & 30 & 66.99 & 6.93& 3.08 & 12 & 11 & 15 - 25 & 7.6 & 4.0 & 17.3 - 7.3\\
      \end{tabular}
    \label{table_28000K}
%  \end{threeparttable}
%\end{adjustwidth}
\end{table*}


\begin{table*}
%\begin{adjustwidth}{-.5in}{-.5in}
%\renewcommand{\arraystretch}{1.1}
    \centering
 % \begin{threeparttable}
    \caption{Table \ref{table_28000K} continued.}
     \begin{tabular}{cccccccccccc}
        \hline \hline
        $M_{\text{OB}}$  & $T_{\text{eff,OB}}$ & $f_{\text{OB}}/f_{\text{tot}}$ & $f_{\text{1}}/f_{\text{tot}}$ & $f_{\text{2}}/f_{\text{tot}}$ &  $T_{\text{eff,1}}$ & $T_{\text{eff,2}}$ & $T_{\text{eff,out}}$  & $M_{\text{1}}$  & $M_{\text{2}}$ & $M_{\text{out}}$ \\
        
        [$M_{\odot}$] & [kK]&[\%]&  [\%]&  [\%]&  [kK]& [kK]&  [kK] &  [$M_{\odot}$] &[$M_{\odot}$] & [$M_{\odot}$]\\
        \hline
        15.0 & 30 & 66.99 & 7.70& 2.31 & 12 & 11 & 15 - 25 & 8.5 & 3.0 & 17.3 - 7.3\\
        15.0 & 30 & 67.76 & 6.16& 3.08 & 12 & 10 & 15 - 25 & 6.7 & 4.8 & 17.1 - 7.3\\
        15.0 & 30 & 68.53 & 5.39& 3.08 & 11 & 10 & 15 - 25 & 6.9 & 4.8 & 17.0 - 7.2\\
        16.0 & 30 & 65.45 & 9.24 & 2.31 & 13 & 12 & 15 - 25&9.7& 2.8& 18.9 - 8.0 \\
        16.0 & 30 & 65.45 & 9.24 & 2.31 & 14 & 10 & 15 - 25&8.5& 4.0& 18.9 - 8.0 \\
        16.0 & 30 & 65.45 & 10.01 & 1.54 & 13 & 12 & 15 - 25 &10.5 & 1.9 & 18.9- 8.0\\
        16.0 & 30 & 66.99 & 6.93& 3.08 & 12 & 11 & 15 - 25 & 8.2 & 4.3 & 18.5 - 7.8\\
        16.0 & 30 & 66.99 & 7.70& 2.31 & 12 & 11 & 15 - 25 & 9.1 & 3.2 & 18.5 - 7.8\\
        16.0 & 30 & 67.76 & 6.16& 3.08 & 12 & 10 & 15 - 25 &7.2 & 5.1 & 18.3 - 7.7\\
        16.0 & 30 & 68.53 & 5.39& 3.08 & 11 & 10 & 15 - 25 & 7.4 & 5.1 & 18.1 - 7.7\\
        17.0 & 30 & 65.45 & 9.24 & 2.31 & 13 & 12 & 15 - 25&10.3& 3.0& 20.1 - 8.5 \\
        17.0 & 30 & 65.45 & 9.24 & 2.31 & 14 & 10 & 15 - 25&9.1& 4.2& 20.1 - 8.5 \\
        17.0 & 30 & 65.45 & 10.01 & 1.54 & 13 & 12 & 15 - 25 &11.1 & 2.0 & 20.1 - 8.5\\
        17.0 & 30 & 66.99 & 6.93& 3.08 & 12 & 11 & 15 - 25 & 8.7 & 4.6 & 19.7 - 8.3\\
        17.0 & 30 & 66.99 & 7.70& 2.31 & 12 & 11 & 15 - 25 & 9.7 & 3.4 & 19.7 - 8.3\\
        17.0 & 30 & 67.76 & 6.16& 3.08 & 12 & 10 & 15 - 25 &7.6 & 5.5 & 19.4 - 8.2\\
        17.0 & 30 & 68.53 & 5.39& 3.08 & 11 & 10 & 15 - 25 & 7.8 & 5.4 & 19.2 - 8.1\\
        \hline
        14.0 & 31 & 65.45 & 8.47 & 3.08 & 14 & 12 & 15 - 25&7.3& 3.5& 17.7 - 7.5 \\
        14.0 & 31 & 65.45 & 8.47 & 3.08 & 16 & 10 & 15 - 25&5.9& 5.0& 17.7 - 7.5 \\
        14.0 & 31 & 65.45 & 9.24 & 2.31 & 15 & 10 & 15 - 25&7.1& 3.7& 17.7 - 7.5 \\
        14.0 & 31 & 66.22 & 7.70 & 3.08 & 13 & 12 & 15 - 25 &7.4 & 3.4 & 17.5 - 7.4\\
        14.0 & 31 & 66.22 & 7.70 & 3.08 & 15 & 10 & 15 - 25 & 5.9 & 4.9 & 17.5 - 7.4\\
        14.0 & 31 & 66.22 & 8.47& 2.31 & 13 & 12 & 15 - 25 & 8.2 & 2.6 & 17.5 - 7.4\\
        14.0 & 31 & 66.22 & 8.47& 2.31 & 14 & 10 & 15 - 25 & 7.2 & 3.7 & 17.5 - 7.4\\
        14.0 & 31 & 66.22 & 9.24& 1.54 & 13 & 11 & 15 - 25 & 9.0 & 2.0 & 17.5 - 7.4\\
        14.0 & 31 & 67.76 & 5.39& 3.85 & 12 & 11 & 15 - 25 & 5.9 & 5.0 & 17.3 - 7.3\\
        14.0 & 31 & 66.22 & 9.24& 1.54 & 13 & 11 & 15 - 25 & 9.0 & 2.0 & 17.1 - 7.3\\
        14.0 & 31 & 67.76 & 7.70& 1.54 & 12 & 11 & 15 - 25 & 8.4 & 2.4 & 17.1 - 7.3\\
        14.0 & 31 & 68.53 & 4.62& 3.85 & 11 & 11 & 15 - 25 & 5.9 & 4.9 & 16.9 - 7.2\\
        14.0 & 31 & 68.53 & 5.39& 3.08 & 11 & 11 & 15 - 25 & 6.9 & 3.9 & 16.9 - 7.2\\
        14.0 & 31 & 68.53 & 6.16& 2.31 & 11 & 11 & 15 - 25 & 7.9 & 3.0 & 16.9 - 7.2\\
        14.0 & 31 & 68.53 & 6.93& 1.54 & 11 & 11 & 15 - 25 & 8.9 & 2.0 & 16.9 - 7.2\\
        15.0 & 31 & 65.45 & 8.47 & 3.08 & 14 & 12 & 15 - 25&7.8& 3.7& 19.0 - 8.0 \\
        15.0 & 31 & 65.45 & 8.47 & 3.08 & 16 & 10 & 15 - 25&6.3& 5.4& 19.0 - 8.0 \\
        15.0 & 31 & 65.45 & 9.24 & 2.31 & 15 & 10 & 15 - 25&7.6& 4.0& 19.0 - 8.0 \\
        15.0 & 31 & 66.22 & 7.70 & 3.08 & 13 & 12 & 15 - 25 &8.0 & 3.7 & 18.8 - 8.0\\
        15.0 & 31 & 66.22 & 7.70 & 3.08 & 15 & 10 & 15 - 25 & 6.3 & 5.3 & 18.8 - 8.0\\
        15.0 & 31 & 66.22 & 8.47& 2.31 & 13 & 12 & 15 - 25 & 8.8 & 2.8 & 18.8 - 8.0\\
        15.0 & 31 & 66.22 & 8.47& 2.31 & 14 & 10 & 15 - 25 & 7.8 & 4.0 & 18.8 - 8.0\\
        15.0 & 31 & 66.22 & 9.24& 1.54 & 13 & 11 & 15 - 25 & 9.6 & 2.2 & 18.8 - 8.0\\
        15.0 & 31 & 67.76 & 5.39& 3.85 & 12 & 11 & 15 - 25 & 6.3 & 5.4 & 18.6 - 7.9\\
        15.0 & 31 & 66.22 & 9.24& 1.54 & 13 & 11 & 15 - 25 & 6.3 & 5.3 & 18.4 - 7.8\\
        15.0 & 31 & 67.76 & 7.70& 1.54 & 12 & 11 & 15 - 25 & 9.0 & 2.6 & 18.4 - 7.8\\
        15.0 & 31 & 68.53 & 4.62& 3.85 & 11 & 11 & 15 - 25 & 6.3 & 5.3 & 18.2 - 7.7\\
        15.0 & 31 & 68.53 & 5.39& 3.08 & 11 & 11 & 15 - 25 & 7.4 & 4.2 & 18.2 - 7.7\\
        15.0 & 31 & 68.53 & 6.16& 2.31 & 11 & 11 & 15 - 25 & 8.4 & 3.2 & 18.2 - 7.7\\
        15.0 & 31 & 68.53 & 6.93& 1.54 & 11 & 11 & 15 - 25 & 9.5 & 2.1 & 18.2 - 7.7\\
       \hline
     \end{tabular}
\end{table*}  

\begin{table*}
%\begin{adjustwidth}{-.5in}{-.5in}
%\renewcommand{\arraystretch}{1.1}
    \centering
 % \begin{threeparttable}
    \caption{Table \ref{table_28000K} continued.}
     \begin{tabular}{cccccccccccc}
        \hline \hline
        $M_{\text{OB}}$  & $T_{\text{eff,OB}}$ & $f_{\text{OB}}/f_{\text{tot}}$ & $f_{\text{1}}/f_{\text{tot}}$ & $f_{\text{2}}/f_{\text{tot}}$ &  $T_{\text{eff,1}}$ & $T_{\text{eff,2}}$ & $T_{\text{eff,out}}$  & $M_{\text{1}}$  & $M_{\text{2}}$ & $M_{\text{out}}$ \\
        
        [$M_{\odot}$] & [kK]&[\%]&  [\%]&  [\%]&  [kK]& [kK]&  [kK] &  [$M_{\odot}$] &[$M_{\odot}$] & [$M_{\odot}$]\\
        \hline
        16.0 & 31 & 65.45 & 8.47 & 3.08 & 14 & 12 & 15 - 25&8.4& 4.0& 20.3 - 8.6 \\
        16.0 & 31 & 65.45 & 8.47 & 3.08 & 16 & 10 & 15 - 25&6.7& 5.7& 20.3 - 8.6 \\
        16.0 & 31 & 65.45 & 9.24 & 2.31 & 15 & 10 & 15 - 25&8.1& 4.3& 20.3 - 8.6 \\
        16.0 & 31 & 66.22 & 7.70 & 3.08 & 13 & 12 & 15 - 25 &8.5 & 3.9 & 20.0 - 8.5\\
        16.0 & 31 & 66.22 & 7.70 & 3.08 & 15 & 10 & 15 - 25 & 6.7 & 5.6 & 20.0 - 8.5\\
        16.0 & 31 & 66.22 & 8.47& 2.31 & 13 & 12 & 15 - 25 & 9.4 & 3.0 & 20.0 - 8.5\\
        16.0 & 31 & 66.22 & 8.47& 2.31 & 14 & 10 & 15 - 25 & 8.3 & 4.2 & 20.0 - 8.5\\
        16.0 & 31 & 66.22 & 9.24& 1.54 & 13 & 11 & 15 - 25 & 10.2 & 2.3 & 20.0 - 8.5\\
        16.0 & 31 & 67.76 & 5.39& 3.85 & 12 & 11 & 15 - 25 & 6.7 & 5.8 & 19.8 - 8.4\\
        16.0 & 31 & 66.22 & 9.24& 1.54 & 13 & 11 & 15 - 25 & 6.7 & 5.7 & 19.6 - 8.3\\
        16.0 & 31 & 67.76 & 7.70& 1.54 & 12 & 11 & 15 - 25 & 9.6 & 2.8 & 19.6 - 8.3\\
        16.0 & 31 & 68.53 & 4.62& 3.85 & 11 & 11 & 15 - 25 & 6.7 & 5.6 & 19.4 - 8.2\\
        16.0 & 31 & 68.53 & 5.39& 3.08 & 11 & 11 & 15 - 25 & 7.9 & 4.5 & 19.4 - 8.2\\
        16.0 & 31 & 68.53 & 6.16& 2.31 & 11 & 11 & 15 - 25 & 9.0 & 3.4 & 19.4 - 8.2\\
        16.0 & 31 & 68.53 & 6.93& 1.54 & 11 & 11 & 15 - 25 & 10.1 & 2.2 & 19.4 - 8.2\\
        17.0 & 31 & 65.45 & 8.47 & 3.08 & 14 & 12 & 15 - 25&8.9& 4.2& 21.5 - 9.1\\
        17.0 & 31 & 65.45 & 8.47 & 3.08 & 16 & 10 & 15 - 25&7.1& 6.1& 21.5 - 9.1 \\
        17.0 & 31 & 65.45 & 9.24 & 2.31 & 15 & 10 & 15 - 25&8.7& 4.5& 21.5 - 9.1 \\
        17.0 & 31 & 66.22 & 7.70 & 3.08 & 13 & 12 & 15 - 25 &9.1 & 4.2 & 21.3 - 9.0\\
        17.0 & 31 & 66.22 & 7.70 & 3.08 & 15 & 10 & 15 - 25 & 7.1 & 6.0 & 21.3 - 9.0\\
        17.0 & 31 & 66.22 & 8.47& 2.31 & 13 & 12 & 15 - 25 &10.0& 3.1 & 21.3 - 9.0\\
        17.0 & 31 & 66.22 & 8.47& 2.31 & 14 & 10 & 15 - 25 & 8.8 & 4.5 & 21.3 - 9.0\\
        17.0 & 31 & 66.22 & 9.24& 1.54 & 13 & 11 & 15 - 25 & 10.9& 2.5 & 21.3 - 9.0\\
        17.0 & 31 & 67.76 & 5.39& 3.85 & 12 & 11 & 15 - 25 & 7.2 & 6.0& 21.0 - 8.9\\
        17.0 & 31 & 66.22 & 9.24& 1.54 & 13 & 11 & 15 - 25 & 7.2 & 6.0 & 20.8 - 8.8\\
        17.0 & 31 & 67.76 & 7.70& 1.54 & 12 & 11 & 15 - 25 & 10.2 & 2.9 & 20.8 - 8.8\\
        17.0 & 31 & 68.53 & 4.62& 3.85 & 11 & 11 & 15 - 25 & 7.2 & 6.0 & 20.6 - 8.7\\
        17.0 & 31 & 68.53 & 5.39& 3.08 & 11 & 11 & 15 - 25 & 8.4 & 4.8 & 20.6 - 8.7\\
        17.0 & 31 & 68.53 & 6.16& 2.31 & 11 & 11 & 15 - 25 & 9.6 & 3.6 & 20.6 - 8.7\\
        17.0 & 31 & 68.53 & 6.93& 1.54 & 11 & 11 & 15 - 25 & 10.8 & 2.4 & 20.6 - 8.7\\
        \hline
        14.0 & 32 & 65.45 & 7.70 & 3.85 & 15 & 12 & 15 - 25&6.3& 4.7& 18.9 - 8.0 \\
        14.0 & 32 & 65.45 & 9.24 & 2.31 & 14 & 13 & 15 - 25&8.5& 2.4& 18.9 - 8.0 \\
        14.0 & 32 & 65.45 & 9.24 & 2.31 & 15 & 11 & 15 - 25&7.6& 3.3& 18.9 - 8.0 \\
        14.0 & 32 & 65.45 & 9.24 & 2.31 & 16 & 10 & 15 - 25&6.8& 4.0& 18.9 - 8.0 \\
        14.0 & 32 & 65.45 & 10.01 & 1.54 & 14 & 13 & 15 - 25&9.2& 1.6 & 18.9 - 8.0 \\
        14.0 & 32 & 65.45 & 10.01 & 1.54 & 15 & 10 & 15 - 25&8.2& 2.7& 18.9 - 8.0 \\
        14.0 & 32 & 66.22 & 6.93 & 3.85 & 14 & 12 & 15 - 25&6.3& 4.6& 18.7 - 7.9 \\
        14.0 & 32 & 66.22 & 7.70 & 3.08 & 16 & 10 & 15 - 25&5.6& 5.3& 18.7 - 7.9 \\
        14.0 & 32& 66.22 & 8.47 & 2.31 & 14 & 11 & 15 - 25&7.7& 3.3& 18.7 - 7.9 \\
        14.0 & 32 & 66.22 & 8.47 & 2.31 & 15 & 10 & 15 - 25&6.9& 3.9& 18.7 - 7.9 \\
        14.0 & 32 & 66.99 & 5.39 & 4.62 & 13 & 12 & 15 - 25&5.5& 5.5& 18.5 - 7.8 \\
        14.0 & 32 & 66.99 & 6.16 & 3.85 & 13 & 12 & 15 - 25&6.3& 4.5& 18.5 - 7.8 \\
        14.0 & 32 & 66.99 & 6.16 & 3.85 & 14 & 11 & 15 - 25&5.5& 5.4& 18.5 - 7.8 \\
        14.0 & 32 & 66.99 & 7.70 & 2.31 & 14 & 10 & 15 - 25&6.9& 3.9& 18.5 - 7.8 \\
        14.0 & 32 & 66.99 & 8.47 & 1.54 & 13 & 11 & 15 - 25&8.7& 2.1& 18.5 - 7.8 \\
        14.0 & 32 & 67.76 & 4.62 & 4.62 & 12 & 12 & 15 - 25&5.4& 5.4& 18.3 - 7.7 \\
        14.0 & 32 & 67.76 & 5.39 & 3.85 & 12 & 12 & 15 - 25&6.3& 4.5& 18.3 - 7.7 \\
        14.0 & 32 & 67.76 & 6.16 & 3.08 & 12 & 12 & 15 - 25&7.2& 3.6& 18.3 - 7.7 \\
        \hline
    \end{tabular}
    \label{table_31000K}
%  \end{threeparttable}
%\end{adjustwidth}
\end{table*}

\begin{table*}
%\begin{adjustwidth}{-.5in}{-.5in}
%\renewcommand{\arraystretch}{1.1}
    \centering
 % \begin{threeparttable}
    \caption{Table \ref{table_28000K} continued.}
     \begin{tabular}{cccccccccccc}
        \hline \hline
        $M_{\text{OB}}$  & $T_{\text{eff,OB}}$ & $f_{\text{OB}}/f_{\text{tot}}$ & $f_{\text{1}}/f_{\text{tot}}$ & $f_{\text{2}}/f_{\text{tot}}$ &  $T_{\text{eff,1}}$ & $T_{\text{eff,2}}$ & $T_{\text{eff,out}}$  & $M_{\text{1}}$  & $M_{\text{2}}$ & $M_{\text{out}}$ \\
        
        [$M_{\odot}$] & [kK]&[\%]&  [\%]&  [\%]&  [kK]& [kK]&  [kK] &  [$M_{\odot}$] &[$M_{\odot}$] & [$M_{\odot}$]\\
        \hline
        14.0 & 32 & 67.76 & 6.93 & 2.31 & 12 & 12 & 15 - 25&8.1& 2.7& 18.3 - 7.7 \\
        14.0 & 32& 67.76 & 6.93 & 2.315 & 13 & 10 & 15 - 25&7.0& 3.9& 18.3 - 7.7 \\
        14.0 & 32 & 67.76 & 7.70 & 1.54 & 12 & 12 & 15 - 25&9.0& 1.8& 18.3 - 7.7 \\
        14.0 & 32 & 68.53 & 6.16 & 2.31 & 12 & 10 & 15 - 25&7.1& 3.8& 18.0 - 7.6 \\
        14.0 & 32 & 69.30 & 6.16 & 1.54 & 11 & 10 & 15 - 25&8.3& 2.5& 17.8 - 7.6 \\
        15.0 & 32 & 65.45 & 7.70 & 3.85 & 15 & 12 & 15 - 25&6.8& 5.0& 20.3 - 8.6 \\
        15.0 & 32 & 65.45 & 9.24 & 2.31 & 14 & 13 & 15 - 25&9.1& 2.6& 20.3 - 8.6 \\
        15.0 & 32 & 65.45 & 9.24 & 2.31 & 15 & 11 & 15 - 25&8.1& 3.5 & 20.3 - 8.6 \\
        15.0 & 32 & 65.45 & 9.24 & 2.31 & 16 & 10 & 15 - 25&7.3& 4.3& 20.3 - 8.6 \\
        15.0 & 32 & 65.45 & 10.01 & 1.54 & 14 & 13 & 15 - 25&9.9& 1.7 & 20.3 - 8.6 \\
        15.0 & 32 & 65.45 & 10.01 & 1.54 & 15 & 10 & 15 - 25&8.8& 2.9& 20.3 - 8.6 \\
        15.0 & 32 & 66.22 & 6.93 & 3.85 & 14 & 12 & 15 - 25&6.8& 4.9& 20.0 - 8.5 \\
        15.0 & 32 & 66.22 & 7.70 & 3.08 & 16 & 10 & 15 - 25&6.0& 5.6& 20.0 - 8.5 \\
        15.0 & 32 & 66.22 & 8.47 & 2.31 & 14 & 11 & 15 - 25&8.3& 3.5& 20.0 - 8.5 \\
        15.0 & 32 & 66.22 & 8.47 & 2.31 & 15 & 10 & 15 - 25&7.4& 4.2& 20.0 - 8.5 \\
        15.0 & 32 & 66.99 & 5.39 & 4.62 & 13 & 12 & 15 - 25&5.9& 5.8& 19.8 - 8.4 \\
        15.0 & 32 & 66.99 & 6.16 & 3.85 & 13 & 12 & 15 - 25&6.7& 4.9& 19.8 - 8.4 \\
        15.0 & 32 & 66.99 & 6.16 & 3.85 & 14 & 11 & 15 - 25&5.9& 5.8& 19.8 - 8.4 \\
        15.0 & 32 & 66.99 & 7.70 & 2.31 & 14 & 10 & 15 - 25&7.4& 4.2& 19.8 - 8.4 \\
        15.0 & 32 & 66.99 & 8.47 & 1.54 & 13 & 11 & 15 - 25&9.3& 2.3& 19.8 - 8.4 \\
        15.0 & 32 & 67.76 & 4.62 & 4.62 & 12 & 12 & 15 - 25&5.8& 5.8& 19.6 - 8.3 \\
        15.0 & 32 & 67.76 & 5.39 & 3.85 & 12 & 12 & 15 - 25&6.7& 4.8& 19.6 - 8.3 \\
        15.0 & 32 & 67.76 & 6.16 & 3.08 & 12 & 12 & 15 - 25&7.7& 3.9& 19.6 - 8.3 \\
        15.0 & 32 & 67.76 & 6.93 & 2.31 & 12 & 12 & 15 - 25&8.7& 2.9& 19.6 - 8.3 \\
        15.0 & 32 & 67.76 & 6.93 & 2.315 & 13 & 10 & 15 - 25&7.5& 4.1& 19.6 - 8.3 \\
        15.0 & 32 & 67.76 & 7.70 & 1.54 & 12 & 12 & 15 - 25&9.6& 1.9& 19.6 - 8.3 \\
        15.0 & 32 & 68.53 & 6.16 & 2.31 & 12 & 10 & 15 - 25&7.6& 4.1& 19.4 - 8.2 \\
        15.0 & 32 & 69.30 & 6.16 & 1.54 & 11 & 10 & 15 - 25&8.9& 2.7& 19.1 - 8.1 \\
        16.0 & 32 & 65.45 & 7.70 & 3.85 & 15 & 12 & 15 - 25&7.2& 5.3& 21.6 - 9.2 \\
        16.0 & 32 & 65.45 & 9.24 & 2.31 & 14 & 13 & 15 - 25&9.7& 2.8& 21.6 - 9.2 \\
        16.0 & 32 & 65.45 & 9.24 & 2.31 & 15 & 11 & 15 - 25&8.7& 3.8 & 21.6 - 9.2 \\
        16.0 & 32 & 65.45 & 9.24 & 2.31 & 16 & 10 & 15 - 25&7.8& 4.6& 21.6 - 9.2 \\
        16.0 & 32 & 65.45 & 10.01 & 1.54 & 14 & 13 & 15 - 25&10.5& 1.8 & 21.6 - 9.2 \\
        16.0 & 32 & 65.45 & 10.01 & 1.54 & 15 & 10 & 15 - 25&9.4& 3.0& 21.6 - 9.2 \\
        16.0 & 32 & 66.22 & 6.93 & 3.85 & 14 & 12 & 15 - 25&7.2& 5.3& 21.4 - 9.0 \\
        16.0 & 32 & 66.22 & 7.70 & 3.08 & 16 & 10 & 15 - 25&6.4& 6.0& 21.4 - 9.0 \\
        16.0 & 32 & 66.22 & 8.47 & 2.31 & 14 & 11 & 15 - 25&8.8& 3.7& 21.4 - 9.0 \\
        16.0 & 32 & 66.22 & 8.47 & 2.31 & 15 & 10 & 15 - 25&7.9& 4.5& 21.4 - 9.0 \\
        16.0 & 32 & 66.99 & 5.39 & 4.62 & 13 & 12 & 15 - 25&6.3& 6.2& 21.1 - 8.9 \\
        16.0 & 32 & 66.99 & 6.16 & 3.85 & 13 & 12 & 15 - 25&7.2& 5.2& 21.1 - 8.9 \\
        16.0 & 32 & 66.99 & 6.16 & 3.85 & 14 & 11 & 15 - 25&6.3& 6.1& 21.1 - 8.9 \\
        16.0 & 32 & 66.99 & 7.70 & 2.31 & 14 & 10 & 15 - 25&7.9& 4.5& 21.1 - 8.9 \\
        16.0 & 32 & 66.99 & 8.47 & 1.54 & 13 & 11 & 15 - 25&9.9& 2.5& 21.1 - 8.9 \\
        16.0 & 32 & 67.76 & 4.62 & 4.62 & 12 & 12 & 15 - 25&6.2& 6.2& 20.9 - 8.8 \\
        16.0 & 32 & 67.76 & 5.39 & 3.85 & 12 & 12 & 15 - 25&7.2& 5.1& 20.9 - 8.8 \\
        16.0 & 32 & 67.76 & 6.16 & 3.08 & 12 & 12 & 15 - 25&8.2& 4.1& 20.9 - 8.8 \\
        16.0 & 32 & 67.76 & 6.93 & 2.31 & 12 & 12 & 15 - 25&9.2& 3.1& 20.9 - 8.8 \\
        16.0 & 32 & 67.76 & 6.93 & 2.315 & 13 & 10 & 15 - 25&8.0& 4.4& 20.9 - 8.8 \\
        \hline
    \end{tabular}
    \label{table_31000K}
%  \end{threeparttable}
%\end{adjustwidth}
\end{table*}

\begin{table*}
%\begin{adjustwidth}{-.5in}{-.5in}
%\renewcommand{\arraystretch}{1.1}
    \centering
 % \begin{threeparttable}
    \caption{Table \ref{table_28000K} continued.}
     \begin{tabular}{cccccccccccc}
        \hline \hline
        $M_{\text{OB}}$  & $T_{\text{eff,OB}}$ & $f_{\text{OB}}/f_{\text{tot}}$ & $f_{\text{1}}/f_{\text{tot}}$ & $f_{\text{2}}/f_{\text{tot}}$ &  $T_{\text{eff,1}}$ & $T_{\text{eff,2}}$ & $T_{\text{eff,out}}$  & $M_{\text{1}}$  & $M_{\text{2}}$ & $M_{\text{out}}$ \\
        
        [$M_{\odot}$] & [kK]&[\%]&  [\%]&  [\%]&  [kK]& [kK]&  [kK] &  [$M_{\odot}$] &[$M_{\odot}$] & [$M_{\odot}$]\\
        \hline
        16.0 & 32 & 67.76 & 7.70 & 1.54 & 12 & 12 & 15 - 25&10.3& 2.1& 20.9 - 8.8 \\
        16.0 & 32 & 68.53 & 6.16 & 2.31 & 12 & 10 & 15 - 25&8.1& 4.4& 20.6 - 8.7 \\
        16.0 & 32 & 69.30 & 6.16 & 1.54 & 11 & 10 & 15 - 25&9.5& 2.9& 20.4 - 8.6 \\
        17.0 & 32 & 65.45 & 7.70 & 3.85 & 15 & 12 & 15 - 25&7.7& 5.6& 23.0 - 9.7 \\
        17.0 & 32 & 65.45 & 9.24 & 2.31 & 14 & 13 & 15 - 25&10.3& 2.9& 23.0 - 9.7 \\
        17.0 & 32 & 65.45 & 9.24 & 2.31 & 15 & 11 & 15 - 25&9.2& 4.0 & 23.0 - 9.7 \\
        17.0 & 32 & 65.45 & 9.24 & 2.31 & 16 & 10 & 15 - 25&8.3& 4.8& 23.0 - 9.7 \\
        17.0 & 32 & 65.45 & 10.01 & 1.54 & 14 & 13 & 15 - 25&11.2& 2.0 & 23.0 - 9.7 \\
        17.0 & 32 & 65.45 & 10.01 & 1.54 & 15 & 10 & 15 - 25&10.0& 3.2& 23.0 - 9.7 \\
        17.0 & 32 & 66.22 & 6.93 & 3.85 & 14 & 12 & 15 - 25&7.7& 5.6& 22.7 - 9.6 \\
        17.0 & 32 & 66.22 & 7.70 & 3.08 & 16 & 10 & 15 - 25&6.8& 6.4& 22.7 - 9.6 \\
        17.0 & 32 & 66.22 & 8.47 & 2.31 & 14 & 11 & 15 - 25&9.4& 4.0& 22.7 - 9.6 \\
        17.0 & 32 & 66.22 & 8.47 & 2.31 & 15 & 10 & 15 - 25&8.4& 4.8& 22.7 - 9.6 \\
        17.0 & 32 & 66.99 & 5.39 & 4.62 & 13 & 12 & 15 - 25&6.7& 6.6& 22.4 - 9.5 \\
        17.0 & 32 & 66.99 & 6.16 & 3.85 & 13 & 12 & 15 - 25&7.6& 5.5& 22.4 - 9.5 \\
        17.0 & 32 & 66.99 & 6.16 & 3.85 & 14 & 11 & 15 - 25&6.7& 6.5& 22.4 - 9.5 \\
        17.0 & 32 & 66.99 & 7.70 & 2.31 & 14 & 10 & 15 - 25&8.4& 4.7& 22.4 - 9.5 \\
        17.0 & 32 & 66.99 & 8.47 & 1.54 & 13 & 11 & 15 - 25&10.5& 2.6& 22.4 - 9.5 \\
        17.0 & 32 & 67.76 & 4.62 & 4.62 & 12 & 12 & 15 - 25&6.5& 6.5& 22.2 - 9.4 \\
        17.0 & 32 & 67.76 & 5.39 & 3.85 & 12 & 12 & 15 - 25&7.6& 5.5& 22.2 - 9.4 \\
        17.0 & 32 & 67.76 & 6.16 & 3.08 & 12 & 12 & 15 - 25&8.7& 4.4& 22.2 - 9.4 \\
        17.0 & 32 & 67.76 & 6.93 & 2.31 & 12 & 12 & 15 - 25&9.8& 3.3& 22.2 - 9.4 \\
        17.0 & 32 & 67.76 & 6.93 & 2.315 & 13 & 10 & 15 - 25&8.5& 4.7& 22.2 - 9.4 \\
        17.0 & 32 & 67.76 & 7.70 & 1.54 & 12 & 12 & 15 - 25&10.9& 2.2& 22.2 - 9.4 \\
        17.0 & 32 & 68.53 & 6.16 & 2.31 & 12 & 10 & 15 - 25&8.6& 4.6& 21.9 - 9.3 \\
        17.0 & 32 & 69.30 & 6.16 & 1.54 & 11 & 10 & 15 - 25&10.1& 3.1& 21.7 - 9.2\\
        \hline
    \end{tabular}
    %      \flushleft
    % \begin{tablenotes}
    %   \small
    %   \item \textbf{Notes.} 
    % \end{tablenotes}
    \label{table_31000K}
%  \end{threeparttable}
%\end{adjustwidth}
\end{table*}



==> soetkin.tex <==

We vary the temperature of the O9.5-B0.5V star between 20,000 - 32,000 K. For the two components of the binary companion, effective temperatures were varied between 10,000 - 20,000 K in steps of 1,000 K. While fitting, we assumed that the effective temperature of the secondary component of the binary was smaller or equal to that of the primary. The effective temperature of the outer 0.5" component ranged from 15,000  - 25,000 K. For each component in the system, we assumed $\log g = 4.0$\,dex. In the $V$-band, the contribution of the O9.5-B0.5V + binary system is fixed to 77\%, of which the O9.5-B0.5V contributes between 85-94\%. Hence the binary contributes between 6-15\% of those 77\%. Here, we assumed that the contribution of the primary is again larger or equal to that of the secondary. The contribution of the fourth component was fixed to the remaining 23\%.

Since the distance to the system and the radii of the components are scaling factors for the model SEDs (e.g. when the system is further away, this results in a downwards shift of the whole model), these can be fixed and the fitting will account for any large deviations from reality by shifting the combined model up or down to fit the photometric data, resulting in a multiplication of the model flux or an addition on the logarithmic luminosity. Hence, the luminosity of the O9.5-B0.5V star can be calibrated to an expected value and the luminosities of the other components will scale accordingly. By using the assumption that $\log g = 4.0$\,dex, a radius $R$ can be obtained through $g = GM/R^2$ for every mass $M$ of the O9.5-B0.5V star in the range $14-17\,M_{\odot}$ with a step of $1M_{\odot}$. For a given temperature in the range specified above, a luminosity can be obtained for every $R$. Reversing the calculations, we can obtain a radius for each component from the obtained luminosity, from which a mass can obtained ($\log g = 4.0$\,dex). Finally, the mass ratio of the O9.5-B0.5V star and its binary companion can be obtained. 

Only few combinations of contributions, effective temperatures, and mass of the O9.5-B0.5V star agree with the derived mass ratio of 0.7776. Table \ref{table_28000K} presents those that have a mass ratio within 1\% of the derived one and a mass of the primary which is larger than the mass of the secondary. Although all solutions returned by the fitting are given, several of those can be excluded when taking into account that both components of the binary system are main-sequence stars. Hence, for example, for solutions with a mass of the primary around $7-8M_{\odot}$ and effective temperature of 12\,000\,K, the effective temperature is too low for such a massive star. This results in all solutions with $T_{\text{eff,OB}} = 28-29-30$\,kK to be excluded as possible configurations. The most likely solutions, which satisfy the main-sequence nature of the binary components, are those with binary mass-ratios close to unity, with a primary mass around $5-6M_{\odot}$. Also lower masses of $14-15M_{\odot}$ for the O9.5-B0.5V are favoured. No conclusion can be drawn for the outer 0.5" component.

One of the uncertainties embedded in the fitting is the assumption that the reddening for each of the components is equal. Since it remains uncertain whether or not the 0.5" component is bound to the O9.5-B0.5V + binary system, this might not be the case. Hence, the interpretation of the above stated results should be done with caution.

\textbf{part that belongs in section 3.2:}
Other photometric data include Johnson, Hipparcos, SDSS, 2MASS, and WISE data. These data are listed in Table \ref{table_data_vizier} with their corresponding references. 

% \input{Appendix_Soetkin}
% \input{Table_results_Soetkin}

